Approximate Maximum Matching in Random Streams

In this paper, we study the problem of finding a maximum matching in the semi-streaming model when edges arrive in a random order. In the semi-streaming model, an algorithm receives a stream of edges and it is allowed to have a memory of $\tilde{O}(n)$ where $n$ is the number of vertices in the graph. A recent inspiring work by Assadi et al. shows that there exists a streaming algorithm with the approximation ratio of $\frac{2}{3}$ that uses $\tilde{O}(n^{1.5})$ memory. However, the memory of their algorithm is much larger than the memory constraint of the semi-streaming algorithms. In this work, we further investigate this problem in the semi-streaming model, and we present simple algorithms for approximating maximum matching in the semi-streaming model. Our main results are as follows. We show that there exists a single-pass deterministic semi-streaming algorithm that finds a $\frac{3}{5} (= 0.6)$ approximation of the maximum matching in bipartite graphs using $\tilde{O}(n)$ memory. This result significantly outperforms the state-of-the-art result of Konrad that finds a $0.539$ approximation of the maximum matching using $\tilde{O}(n)$ memory. By giving a black-box reduction from finding a matching in general graphs to finding a matching in bipartite graphs, we show there exists a single-pass deterministic semi-streaming algorithm that finds a $\frac{6}{11} (\approx 0.545)$ approximation of the maximum matching in general graphs, improving upon the state-of-art result $0.506$ approximation by Gamlath et al.

==> old-table-streaming-alg-summary.tex <==

\begin{table}
\centering
%\resizebox{9.5cm}{!}{%
\begin{tabular}{|l|c|c|c|} 
\hline
 &Apx factor & Apx factor & Space \\
& in bipartite graphs & in general graphs & \\
\hline
&&&\\[-0.7em] 
\citeboth{DBLP:conf/soda/KapralovKS14} & $\frac{1}{\pl n}$ & $\frac{1}{\pl n}$ & $O(\pl n)$ \\
\hline
&&&\\[-0.7em] 

\citeboth{DBLP:conf/approx/KonradMM12} & $0.5005$ & $0.5003$ & $\tilde{O}(n)$ \\
\hline
&&&\\[-0.7em] 


\citeboth{DBLP:journals/corr/abs-1811-02760} & $0.512$ & $0.506$ & $\tilde{O}(n)$ \\
\hline
&&&\\[-0.7em] 
 

\citeboth{DBLP:conf/mfcs/Konrad18} & $0.539$ & - & $\tilde{O}(n)$ \\
\hline
&&&\\[-0.7em] 

\textbf{This paper} & $0.6$ & $0.545$ & $\tilde{O}(n)$ \\
\hline
&&&\\[-0.7em] 


\citeboth{DBLP:conf/soda/AssadiBBMS19} & $0.667$ & $0.667$ & $\tilde{O}(n^{1.5})$ \\
\hline
\end{tabular}
%}%
\caption{Streaming algorithms known for the maximum matching when edges arrive in a random order.}
\label{table:relatedwork}
\vspace{-0.1cm}
\end{table}
